MotionGlot: A Multi-Embodied Motion Generation Model

This paper introduces MotionGlot, a model that can generate motion across multiple embodiments with different action dimensions, such as quadruped robots and human bodies. By leveraging the well-established training procedures commonly used in large language models (LLMs), we introduce an instruction-tuning template specifically designed for motionrelated tasks. Our approach demonstrates that the principles underlying LLM training can be successfully adapted to learn a wide range of motion generation tasks across multiple embodiments with different action dimensions. We demonstrate the various abilities of MotionGlot on a set of 6 tasks and report an average improvement of 35.3% across tasks. Additionally, we contribute two new datasets: (1) a dataset of expert-controlled quadruped locomotion with approximately 48,000 trajectories paired with direction-based text annotations, and (2) a dataset of over 23,000 situational text prompts for human motion generation tasks. Finally, we conduct hardware experiments to validate the capabilities of our system in real-world applications.

==> content/text/introduction.tex <==
Here's a rough draft of the intro:

\begin{itemize}
    \item LLMs, trained as next-token predictors, have been hugely successful. Provide examples numbers and some evidence for this statement.
    \item Language/action and motion have some similarities: they are sequential, structured, etc.
    \item Can we apply the same machinery as LLMs for motion generation? Obviously, yes, since previous work has tried to do this.
    \item However, previous work has important limitations: cannot handle multiple embodiments, cannot easily transfer between embodiments, etc.
    \item We propose MotionGlot, a model that enables motion generation ... instruction tuning, etc. ... We can handle multiple modalities.
    \item MotionGlot has some core capabilities: generation motion for embodiment 1, motion for embodiment 2, text-to-emb1/emb2 motion, motion to text (captioning), etc.
    \item MotionGlot also enables new applications such as instruction following, and goal reaching (conditioned generation).
    \item We demonstrate through experiments that our model is better than ...
    \item Contributions: (1) MotionGlot, instruction tuning, (2) multiple applications with a single model (3)~dataset.
\end{itemize}
 




Training autoregressive \textit{Large Language Models} (LLMs) \cite{gpt, gpt-4, gpt2, llama} using next-token prediction has led to two key advantages:\begin{enumerate*}[label=\textbf{(\arabic*)}]
\item \textit{\textbf{Multi-task Learning}:} Next-token prediction is a versatile technique that enables a decoder-only transformer model to be trained across multiple tasks \cite{gpt}.
\item \textit{\textbf{Instruction Following}:} \textit{LLMs} \cite{gpt,gpt2,llama} can be trained to obey natural language instructions\cite{instruction_tune}. \end{enumerate*} Similar to text even motion trajectories are sequential forms of data and just as in language, where the position of each word depends on past content and the intended future sentence, a local segment of a trajectory is shaped by its past motion and the intended future motion. Observing these parallels between language and motion, we ask a question that would bring the advantages of \textit{LLMs} to the field of motion generation in robotics: \textbf{if an \textit{LLM} \cite{gpt-4,gpt2,llama} can operate as a multi-task learner on textual data, can the same machinery (a decoder only transformer) be employed to perform a multitude of tasks and follow user instructions on motion trajectories across different embodiments?}. 


In this paper, we answer the above question by adapting well-established instruction-tuning techniques of \textit{LLMs} to motion data, thereby, unlocking a wide range of motion-related multi-task learning applications. For example, \begin{enumerate*}[label=\textbf{(\arabic*)}] \item   Text-conditioned motion generation can be approached as a machine translation problem, this approach can be further extended to treat semantic skill transfer between different embodiments, such as humans and robots, as a multi-lingual machine translation problem \cite{xglm,gpt,mt5}. \item  LLM-based question-and-answer techniques can be adapted to generate motion based on specific situations. 
\item  Autoregressive models can facilitate goal-conditioned motion generation, while heuristic-based sampling methods can assist in obstacle avoidance. \end{enumerate*} While our insights and framework can be generalized and extended to multiple morphologies, we are primarily interested in functions performed by human bodies and quadruped robots in this work. 


Building a framework for motion generation across morphologies with properties analogous to \textit{LLMs} poses multiple challenges. First, While \cite{rt2,openvla} have attempted to unify language with text, their approach is largely limited to a single embodiment and cannot be trivially extended to a multi-embodied setting. Second, there is a lack of motion data with textual descriptions for quadrupeds bottlenecks its text-conditioned motion generation ability. 
Second, while there exists human motion data \cite{AMASS,humanml,BABEL} the available text description is action-specific and does not provide any situational context within which the action could be performed, therefore, this data would not suffice for situational-based motion generation. 

To overcome the aforementioned issues we leverage well-established instruction techniques from multi-lingual \textit{LLM} training \cite{mala,instruct_template,instruct_template2,instruction_tune} and propose an instruction template to train a GPT for multi-embodied motion generation. Our method employs a decoder-only transformer \cite{gpt2,gpt-4,gpt,llama} which is a generalized framework in comparison to an encoder-decoder \cite{attention,t5}. Furthermore, we curate a dataset of expert-controlled quadruped locomotion with direction-based text annotation, such a dataset would enable to push the boundaries of text-conditioned robot motion generation. To overcome the drawbacks withing \cite{humanml,BABEL} we verage the few-shot learning abilities of \textit{GPT-4} \cite{gpt-4} to create a dataset with more than $\mathbf{23000}$ situational descriptions of human actions, this data would be used for situation-based motion generation.



Overall our contributions are as follows:
\begin{itemize}
    \item Our primary contribution is to bring the instruction following and multi-task learning ability of \textit{LLMs} to the field of robotics using the same LLM machineary and demonstrate its effectiveness on real-world tasks. 
    \item Our proposed instruction tuning template demonstrates that a single decoder-only transformer can generate motion across multiple embodiments and perform $\mathbf{7}$ tasks as a multi-task learner.
    \item  We create datasets of more than $\mathbf{23000}$ situational prompts for human motion and $\mathbf{48000}$ quadruped trajectories (after augmentation) with direction-based textual descriptions for robot motion.
 \end{itemize}
